DF-GNN: Dynamic Fusion Framework for Attention Graph Neural Networks on GPUs

Attention Graph Neural Networks (AT-GNNs), such as GAT and Graph Transformer, have demonstrated superior performance compared to other GNNs. However, existing GNN systems struggle to efficiently train AT-GNNs on GPUs due to their intricate computation patterns. The execution of AT-GNN operations without kernel fusion results in heavy data movement and significant kernel launch overhead, while fixed thread scheduling in existing GNN kernel fusion strategies leads to sub-optimal performance, redundant computation and unbalanced workload. To address these challenges, we propose a dynamic kernel fusion framework, DF-GNN, for the AT-GNN family. DF-GNN introduces a dynamic bi-level thread scheduling strategy, enabling flexible adjustments to thread scheduling while retaining the benefits of shared memory within the fused kernel. DF-GNN tailors specific thread scheduling for operations in AT-GNNs and considers the performance bottleneck shift caused by the presence of super nodes. Additionally, DF-GNN is integrated with the PyTorch framework for high programmability. Evaluations across diverse GNN models and multiple datasets reveal that DF-GNN surpasses existing GNN kernel optimization works like cuGraph and dgNN, with speedups up to $7.0\times$ over the state-of-the-art non-fusion DGL sparse library. Moreover, it achieves an average speedup of $2.16\times$ in end-to-end training compared to the popular GNN computing framework DGL.

==> 6_relatedwork.tex <==
\section{Related Work}

% \stitle{GNN Frameworks.} NeuGraph~\cite{ma2019neugraph} proposes a distributed training framework built to support efficient and scalable GNN training on large graphs. GNNAdvisor~\cite{GNNAdvisor} is an adaptive and efficient runtime system to accelerate various GNN workloads on GPU platforms. FeatGraph~\cite{hu2020featgraph} utilizes the deep learning compiler TVM~\cite{chen2018tvm} and provides a flexible programming interface. fuseGNN~\cite{chen2020fusegnn} develops two abstractions of GNN aggregation: GAS and GAR, applying GAS for graphs with low average degree and GAR for graphs with high average degree.  HyperGef~\cite{yu2023hypergef} designs a framework that proposes efficient kernel fusion paradigms for Hypergraph Neural Networks.
% Seastar~\cite{wu2021seastar} presents a vertex-centric programming model for GNN training on GPU and produces highly efficient fused GPU kernels for forward and backward passes. However, these works implement few optimization for kernel fusion.

\stitle{Sparse GPU kernel.} Sputnik~\cite{gale2020sparse} develops high performance GPU kernels for SpMM and SDDMM based on the compressed sparse row (CSR) format. 
VectorSparse~\cite{chen2021efficient} introduces a novel mapping between the warp tile and the tensor core unit, implementing a structured SpMM kernel on tensor core. Magicube~\cite{li2022efficient} designs a sparse matrix format SR-BCR and develops a high-performance sparse-matrix library for low-precision integers on Tensor cores. 
Ge-spmm~\cite{huang2020ge} introduces the Coalesced Row Caching and Coarse-grained Warp Merging method for SpMM, developing an efficient CSR-based SpMM-like kernel on GPUs. PRedS~\cite{yu2021exploiting} proposes Vectorized Coarse 1-Dimensional Tiling and other optimizations, implementing a high performance SDDMM kernel.

\stitle{Deep learning compilers.} In deep learning, the kernel fusion work is automatically handled by deep learning compiler. Several DL compiler frameworks have been proposed in recent years~\cite{chen2018tvm, ma2020rammer, ye2023sparsetir, zhao2022apollo, niu2021dnnfusion}. TVM~\cite{chen2018tvm} combines graph-level and operator-level optimizations to generate hardware-specific optimized kernel. DNNFusion~\cite{niu2021dnnfusion} designs high-level abstractions for operator fusion and expands fusion opportunities. Apollo~\cite{zhao2022apollo} integrates graph-level node grouping and operator-level loop fusion and designs a just-in-time (JIT) compilation framework. 

% \noindent \textbf{GNN Kernel Fusion.} fuseGNN\cite{chen2020fusegnn} develops two abstractions of GNN aggregation: Gather-ApplyEdge-Scatter (GAS) and Gather-ApplyEdge-Reduce (GAR), and apples GAS for graphs with low average degree and GAR for graphs with high average degree. 
% FusedMM\cite{rahman2021fusedmm} divides popular graph operators into five types of basic operations and design a general-purpose all fused kernel on CPU. 
% dgNN\cite{zhang2022understanding} proposes a unified thread mapping scheme for both vertex and edge-centric operators to enable fusion and reduce IO. 
% TLPGNN\cite{fu2022tlpgnn} proposes a lightweight two-level parallelism paradigm: node-level and feature-level parallelism to avoid atomic operations and enable coalesced memory access within fused kernels. Unfortunately, none of these existing works considers kernel fusion in graph convolutions with intensive edge computation, such as AGNN or GT. Moreover, they employ a fixed thread schedule strategy that remains constant across different steps of the fused kernel.

% Prior works like (\cite{chen2020fusegnn, rahman2021fusedmm, fu2022tlpgnn, wu2021seastar, zhang2022understanding}) focus on classical but simple graph convolutions(like GCN or GAT), typically adopting a vertex-centric programming paradigm to fuse GNN kernels. However, none of these existing works on advanced graph convolutions with DOT-SDDMM. Furthermore, they employ a fixed thread schedule strategy, which remains constant across different steps of the fused kernel.

% \noindent \textbf{Sparse Operator.}




% % kernel fusion的简介（干啥，效果）
% Kernel fusion on GPU is a technique employed to enhance the performance and efficiency of parallel computing tasks. By combining multiple sequential operations into a single, optimized kernel, kernel fusion minimizes memory accesses, reduces intermediate data storage, and improve computation efficiency, thereby improving overall computation speed.
% % kernel fusion在DNN模型中的情况
% % 在传统的DNN模型中，许多paper对kernel fusion进行了详细的研究，其中涉及到了fusion strategy和code autogenerate 等
% In the traditional DNN models, numerous papers have conducted detailed research on kernel fusion, involving aspects such as fusion strategy and code auto-generation. \cite{ma2020rammer,niu2021dnnfusion,zhao2022apollo}
% % kernel fusion在GNN模型中的情况
% % 已有的工作如(123213）均针对于经典的图卷积操作，如GCN和GAT，采用vertex-centric programming的方式来fuse GNN kernel。 然而，none of these existing work 关注拥有DOT-SDDMM的图卷积如GT，且其采用固定的parallel 方案，在fused kernel的不同step始终不变
% However, in the GNN models, due to the sparse operation and dynamic data shape, the kernel fusion is more challenging, resulting in limited existing research. 



==> 8_acknowledge.tex <==
\section{Acknowledgments}

